Automatic HVAC Control with Real-time Occupancy Recognition and Simulation-guided Model Predictive Control in Low-cost Embedded System

Intelligent building automation systems can reduce the energy consumption of heating, ventilation and air-conditioning (HVAC) units by sensing the comfort requirements automatically and scheduling the HVAC operations dynamically. Traditional building automation systems rely on fairly inaccurate occupancy sensors and basic predictive control using oversimplified building thermal response models, all of which prevent such systems from reaching their full potential. Such limitations can now be avoided due to the recent developments in embedded system technologies, which provide viable low-cost computing platforms with powerful processors and sizeable memory storage in a small footprint. As a result, building automation systems can now efficiently execute highly-sophisticated computational tasks, such as real-time video processing and accurate thermal-response simulations. With this in mind, we designed and implemented an occupancy-predictive HVAC control system in a low-cost yet powerful embedded system (using Raspberry Pi 3) to demonstrate the following key features for building automation: (1) real-time occupancy recognition using video-processing and machine-learning techniques, (2) dynamic analysis and prediction of occupancy patterns, and (3) model predictive control for HVAC operations guided by real-time building thermal response simulations (using an on-board EnergyPlus simulator). We deployed and evaluated our system for providing automatic HVAC control in the large public indoor space of a mosque, thereby achieving significant energy savings.

==> model.tex <==
\section{Model}

The number of occupants is denoted by ${O}(t)$ at time $t$. Consider a single-zone model of a building, where the indoor room temperature is denoted by $T_{\rm i}(t)$ and outdoor temperature by $T_{\rm o}(t)$.
Let $Q_{\rm AC}(t)$ be heat transfer from HVAC system, where as $Q(O(t))$ be the heat emitted by occupants.
The temperature change of $T_{\rm i}(t)$ is modeled by 
\begin{equation}
C_{\rm r} \frac{{\rm d} T_{\rm i}(t)}{{\rm d} t} =
\frac{T_{\rm o}(t) - T_{\rm i}(t)}{R_{\rm r}} + Q_{\rm AC}(t) + Q(O(t))
\end{equation}
where $C_{\rm r}$ is the heat capacity of the room, and $R_{\rm r}$ is the thermal resistance of walls in the room.

By Euler method, we discretize time into time slots $(t_1, t_2, ..., t_T)$.
\begin{equation}
C_{\rm r}  (T_{\rm i}(t_i) - T_{\rm i}(t_{i-1})) =
\frac{T_{\rm o}(t_i) - T_{\rm i}(t_i)}{R_{\rm r}} + Q_{\rm AC}(t_i) + Q(O(t_i))
\end{equation}

Let ${\tt E}(Q_{\rm AC}(t))$ be the energy consumption for the HVAC system. Let $H(t)$ be the ambient humidity, $\underline{T}(H(t))$ and $\overline{T}(H(t))$ be the range of comfortable room temperature with respect to the humidity.

Suppose that the data of occupancy, outdoor temperature and ambient humidity are predicted for an interval $T$, denoted by $\big(\hat{O}(t), \hat{T}_{\rm o}(t), \hat{H}(t)\big)_{t=1}^T$. Define an optimization problem of temperature control given predicted data $\big(\hat{O}(t), \hat{T}_{\rm o}(t), \hat{H}(t)\big)_{t=1}^T$ as follows.

\begin{align}
& \min_{\big(Q_{\rm AC}(t)\big)_{t=1}^T}  \quad \sum_{t = 1}^T  {\tt E}(Q_{\rm AC}(t)) \\
& \mbox{subject to} \notag \\
& C_{\rm r} \frac{{\rm d} T_{\rm i}(t)}{{\rm d} t} =
\frac{\hat{T}_{\rm o}(t) - T_{\rm i}(t)}{R_{\rm r}} + Q_{\rm AC}(t) + Q(\hat{O}(t)) \\
& \underline{T}(\hat{H}(t)) \le T_{\rm i}(t) \le \overline{T}(\hat{H}(t)) \mbox{\ if\ } \hat{O}(t) \ge 0
\end{align}


Define several control strategies:
\begin{enumerate}

\item ({\tt MPC}) Model predictive control strategy optimizes $Q_{\rm AC}(t)$ for an interval $T$, based on predicted data $\big(\hat{O}(\tau), \hat{T}_{\rm o}(\tau), \hat{H}(\tau)\big)_{\tau=t}^{T+t}$.

\item ({\tt AHC}) Ad hoc control strategy optimizes each $Q_{\rm AC}(t)$ at time $t$ based on previous decisions $\big(Q_{\rm AC}(\tau)\big)_{\tau<t}$.

\item ({\tt OLC}) Online control strategy optimizes each $Q_{\rm AC}(t)$ at time $t$ that minimizes the worst-case ratio with model predictive control strategy assuming true future data $\big({O}(\tau), {T}_{\rm o}(\tau), {H}(\tau)\big)_{\tau=t}^{T+t}$.

\end{enumerate}

Define a penalty function to measure the effectiveness 
\begin{align}
& \alpha[\big(Q_{\rm AC}(t)\big)_{t=1}^T] \notag \\
\triangleq & \sum_{t = 1}^T  {\tt E}(Q_{\rm AC}(t)) + \rho_1 [T_{\rm i}(t) - \overline{T}(\hat{H}(t)) ]^+ + \rho_2 [\underline{T}(\hat{H}(t)) - T_{\rm i}(t) ]^+
\end{align}


